A Survey of Practical Formal Methods for Security

In today's world, critical infrastructure is often controlled by computing systems. This introduces new risks for cyber attacks, which can compromise the security and disrupt the functionality of these systems. It is therefore necessary to build such systems with strong guarantees of resiliency against cyber attacks. One way to achieve this level of assurance is using formal verification, which provides proofs of system compliance with desired cyber security properties. The use of Formal Methods (FM) in aspects of cyber security and safety-critical systems are reviewed in this article. We split FM into the three main classes: theorem proving, model checking and lightweight FM. To allow the different uses of FM to be compared, we define a common set of terms. We further develop categories based on the type of computing system FM are applied in. Solutions in each class and category are presented, discussed, compared and summarised. We describe historical highlights and developments and present a state-of-the-art review in the area of FM in cyber security. This review is presented from the point of view of FM practitioners and researchers, commenting on the trends in each of the classes and categories. This is achieved by considering all types of FM, several types of security and safety critical systems and by structuring the taxonomy accordingly. The article hence provides a comprehensive overview of FM and techniques available to system designers of security-critical systems, simplifying the process of choosing the right tool for the task. The article concludes by summarising the discussion of the review, focusing on best practices, challenges, general future trends and directions of research within this field.

==> sections/future-research.tex <==
% !TEX root = ../main.tex
\section{Future Research Vision in Relation with Increased Autonomy}
\label{sec:research-programme}
This survey has enabled us to ponder the future of research into FM within security. While there are many fields that would benefit from this research, in this section we focus on autonomy and autonomous systems as they are often both security and safety critical and it can be expected that they will be deployed across the different domains investigated in this survey as artificial intelligence improves. 

The development of trustworthy autonomous systems needs a multidisciplinary approach including systems security, human factors, modelling, development, and deployment. A vision for their future development is a framework for developing autonomous systems with security built into their design. 

To enable this, strong foundations are needed to cover all stages of development and verification, with a holistic view that includes all components of a system. The scientific basis of the framework must identify and address security requirements in the context of compromised platforms and malicious agents. It needs comprehensive models of software, hardware, communications, user interactions, and environments. Models of human behaviour need to cater to social issues and the capacity to deal with information. A taxonomy and library of models need to support the identification and handling of adversaries and threats that affect security, including privacy. Techniques for design, testing, simulation, and proof must take into account not only functionality but real-time properties to ensure responsiveness. Long-term monitoring and reconfiguration of autonomous systems must provide continued security resilience.

% \subsection{Research Programme}\label{sec:research-programme}

Currently, cyber-security, if considered at all, is an afterthought in the design and development of an autonomous system. Developers address aspects of security only at the implementation level, such as dealing with covert channels introduced by caches or buffer flushing. Delaying security analysis leads to higher development costs and makes it difficult even to articulate system security requirements and consider system-level vulnerabilities. Countermeasures to attacks may need functionality inconsistent with the requirements. For example, cryptography has a computational overhead.

Different threats, attacks, and risks are relevant for different types of autonomy, but there are common underlying commonalities considerations. Security breaches may harm people or the environment or they may cause unauthorised exposure of personal data held by the system collected from its surroundings. Attack surfaces include access points, communications, vulnerable components such as sensors, physical access, and user interactions. Artificial intelligence components introduce new challenges: adversarial attacks, malicious training, and detection of misbehaviour when their expected behaviour is not fully understood.

Security can conflict with usability. Intuitive and usable systems are easier to develop by co-design with end-users, addressing their requirements right from the beginning. Thorough human evaluation can identify weak vulnerabilities to human error or insecure “desire path” behaviours resulting from complex procedures or obscure interface options. Evaluation requires an appreciation of human behaviour, and its limitations and capabilities. When systems make unrealistic cognitive demands on users, they find shortcuts to maintain usability. The benefits of secure autonomous systems require that users perceive that the system is trustworthy, usable, functional, and adaptable. Achieving this is easier if we design the system using a human-centred approach.

Current leading research on autonomous systems reflects an absence of support for consideration of security in the design of autonomous systems. There are some early results for cyber-physical systems and autonomous vehicles~\cite{Katzenbeisser&19}, but they are not connected to the state of the art on system design. We believe that FM shall play significant role in development of secure autonomous systems across different domains.

% \subsection*{Future Research Goals and Objectives}

% The goal of future research is to provide the foundations and tools for the formal analysis, testing, and simulation of security and privacy aspects of autonomous systems. This will range from requirements to run-time execution and human interaction, covering all levels of cyber threat, and enabling the creation of security evidence recognised by certification authorities. We could achieve this goal through six objectives:
% \begin{enumerate}
% \item[O1] Define well-founded, clear, and usable terminology and notation to capture security and privacy requirements for autonomy.
% \item[O2] Define a comprehensive taxonomy of threats, adversarial capabilities, and attack vectors for autonomous systems.
% \item[O3] Establish mathematical foundations and modelling approaches for security: incorporate threats, attacks, responsiveness, and human agency (user and adversarial behaviour).
% \item[O4] Develop techniques for proof, analysis, simulation, and testing for the security of autonomous systems, including human-in-the-loop.
% \item[O5] Develop a library of proven secure and usable system architectures.
% \item[O6] Engage autonomous systems stakeholders in all aspects of security.
% \end{enumerate}

==> sections/netcloud.tex <==
\subsubsection{Authentication}
This section presents FM in security verification of authentication.

\subsubsection{Routing}
This section presents FM in security verification of network routing and communication.

\textbf{Cryptographically Sound and Machine-Assisted Verification of Security Protocols:}

When formal methods are used to verify desirable properties of security protocols, the analysis is often performed on models and not the implementation counterparts. As the ultimate goal of the formal analysis is to guarantee that the implementations are secure, it must be ensured that proven properties carry over to the implementations. To bridge the gap between models and their implementation counterparts, Backes et al.\ propose a refinement-based methodology for verifying that security protocol implementations are cryptographically sound~\cite{Backes&03}. To demonstrate their approach, the authors use the PVS theorem prover~\cite{Owre&92} to formally verify a concrete cryptographic protocol~\cite{Backes&02} for ordered secure message transmission. At the time their work was published in 2003, this was the first example ever of machine-aided, cryptographically sound proof of a security protocol in an asynchronous network.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/protocols.tex <==
\subsubsection{Authorization}
This section presents FM in security verification of communication protocols.

\textbf{Formal Verification of OAuth 2.0 using Alloy Framework:} The authors of~\cite{Pai2011} have used a knowledge flow analysis~\cite{Torlak2005} formalisation technique to formalise an abstract flow presented by the OAuth 2.0 authorisation protocol~\cite{Parecki2017}. The authors have further translated their formalisation to the Alloy specification language and used Alloy analyser to analyse the OAuth 2.0. The analysis have been able to discover a known security vulnerability in the OAuth 2.0 protocol, so called credential storage issue~\cite{Argyriou2017} demonstrating the usefulness of formal analysis. In order to achieve this the author have extended the knowledge flow analysis technique by three specific guidelines.

The Guideline 1 specifies that the "knowledge can neither be created nor it can be destroyed but can be transferred from one principle to the other without the loss of knowledge during transfer". The authors have introduced this guideline to ensure that events such as encryption and compression can be taken as a knowledge transfer between entities. This way the compressor unit as well as encryptor unit shall be modelled as principal. Guideline 2 states that the "knowledge once acquired cannot be forgotten but can become obsolete", this way only finite validity units of knowledge require modelling of timing attributes. Finally the Guideline 3 stating that the "Smaller units of knowledge provided that they have the same value for the duration attribute, can be aggregated into a single large unit, provided that for all principals, either a principal knows all the individual units of knowledge of the composite unit or it knows none of the individual units of knowledge of the composite unit".

The authors represent the principals from OAuth 2.0, the Resource owner, resource server, the client and the authorisation server as predicates $R(x):x$, $O(x):x$, $C(x):x$ and $A(x):x$ and define relations as \textbf{Owns} where the principal has full authority over the value, \textbf{Draws} where the principal knows the value at the start of the protocol, \textbf{Computes} where the principal computes the value using other values in its possession and \textbf{Learns} where the principal knows the value due to interaction with some other principal. The author declare this in Alloy and detect the known vulnerability and conclude that the model allows for search for unknown vulnerabilities in the protocol. The work has shown that usage of Alloy could help to detect vulnerabilities in authorisation protocols.

\textbf{Formal analysis of SAML 2.0 Web Browser SSO apps:} The authors of \cite{Armando2008} have used model checking to verify the Google implementation of SAML 2.0 based single sign on (SSO) for applications \cite{Oasis2005}. Firstly the authors have shown formalisation of the SAML SSO protocol using labeled transition system (LTS) and expressing linear temporal logic (LTL) formulae as constraints on the model. The security aspect addressed in the work is the authentication assertions as defined in the SAML 2.0, specifically it aims at verifying that the security properties of the protocol hold even in case of interference from a malicious attacker. The authors recast the problem to a form $M \models (C_{I} \Rightarrow G)$, where $M$ is a labeled transition system modelling the behaviour of the system including the intruder, $C_{I}$ represents LTL constraints constraining the behaviour of the intruder and $G$ is an LTL property representing the security property of the protocol.

The formalisation have been used to model honest principals as well as intruders. The initial state of the system defines the initial knowledge of the intruder and the model allows for evolution of knowledge throughout the protocol sessions. The model have considered a finite state of protocol sessions. The abilities of the intruder are modelled based on standard Dolev-Yao attacker \cite{Dolev1983}. This allows the attacker to impersonate a honest participant or intercept communication between participants.

The formalisation have been further used to model the communication channels. The authors have defined four types of channels: \textit{1.} The confidential channels where channel $ch$ provides confidentiality only if it is considered an exclusive one to one communication to receiver $p$. \textit{2.} the authentic channels where the input to the channel is accessible exclusively from a single sender. \textit{3.} weakly confidential channels where the output is exclusively open to a single, but unknown receiver. \textit{4.} weakly authentic channels where the exclusively open for single, yet unknown sender. The weakly confidential and weakly authentic channels can be considered channels where one of the principals does not have a valid TLS certificate.

The security properties concerning Authentication and Secrecy have been specified by the authors and verified using the SATMC model checker. The analysis has uncovered a previously unknown vulnerability in the SAML 2.0 protocol implementation where an authentication assertion could be used to spoof identity of a principal. The vulnerability has been reported and a mitigation developed. The work has demonstrated usefulness of model checking in finding unknown vulnerabilities in standard protocols.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

